Employing Gaussian process priors for studying spatial variation in the parameters of a cardiac action potential model

Cardiac cells exhibit variability in the shape and duration of their action potentials in space within a single individual. To create a mathematical model of cardiac action potentials (AP) which captures this spatial variability and also allows for rigorous uncertainty quantification regarding within-tissue spatial correlation structure, we developed a novel hierarchical Bayesian model making use of a latent Gaussian process prior on the parameters of a simplified cardiac AP model which is used to map forcing behavior to observed voltage signals. This model allows for prediction of cardiac electrophysiological dynamics at new points in space and also allows for reconstruction of surface electrical dynamics with a relatively small number of spatial observation points. Furthermore, we make use of Markov chain Monte Carlo methods via the Stan modeling framework for parameter estimation. We employ a synthetic data case study oriented around the reconstruction of a sparsely-observed spatial parameter surface to highlight how this approach can be used for spatial or spatiotemporal analyses of cardiac electrophysiology.

==> older.tex <==

% For literature review non-Bayesian 

\begin{itemize}

\item \cite{Fabri2017} Applied automatic optimization to reduce model discrepancy between experimental data and the Severi-Di Francesco cardiac action potential model and to fit recorded APs and cytosolic calcium transient traces.

\item \cite{Dokos2004} Used Least-squares optimization by curvilinear gradient to perform parameter estimation using the Beeler-Reuter ionic equations for the ventricular action potential.

\item \cite{Sobie2009} used multivariate regression to study parameter sensitivity analysis in electrophysiological models.

\item \cite{Zaniboni2010} Applied a least square iterative method on the Luo Rudy phase I equation system to derive two different sets of parameters that generate two almost identical AP profiles. 
 
\item \cite{Mann2015} used a global optimization approach to improve three existing different action potential models and reproduce clinical data sets more closely by recalibrating the models.  

\item \cite{Krogh2017} Using a human ventricular myocyte model, they show that model optimization to clinical long QT data constrains model parameters in a satisfactory manner using certain bounding intracellular calcium and sodium concentrations.

 \item \cite{Cairns2017} used a genetic algorithm to parameterize cardiac action potential models.
 
 \end{itemize} 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Probability model}
We formulate the dynamics of cardiac action potential modeled in space 
%\al{I think this first part does not make sense} \chris{I'm not sure what you mean; can you clarify here?} 
as a hierarchical Bayesian model for the spatiotemporal action potential function $f(\bm{s}, t)$ where $\bm{s}\in \mathcal{D} \subset  \mathbb{R}^2$ denotes one of $N$ spatial locations located within spatial domain $\mathcal{D}$ and $t$ denotes a temporal coordinate. For simplicity, we assume that the observations are  indexed temporally to an integer-valued grid $t\in \{1,...,T\}$. We let $\bm{U}$ denote the $N\times T$ matrix of voltage observations and $\bm{u}_i$ denotes the $T$-vector of voltages recorded at the time points $1,...,T$ at a single point in space. For each site, a separate Mitchell-Schaeffer ODE model $f_{\bm{\tau}}:\mathbb{R}^T\rightarrow \mathbb{R}^T$ is instantiated with its own set of parameters $\bm{\tau}_i$ to be estimated from the data, though we use a hierarchical prior to share information in space. %Additionally, an external forcing voltage must be applied to drive the system dynamics; we let $x_{it}$ denote the forcing for the $i$-th spatial site at time $t$ and $\bm{x}_i$ denotes the forcing over all time for a single site. 
\al{I am not sure we should talk about the stimulus here}
\chris{We want to make a complete specification for the probability model, and if the stimulus is an input, we should clarify exactly how it fits into the rest of the model. Thus, we do need to describe it in this section.}
Since the MS model has 5 five free parameters and a single noise parameter, we note that $M=\vert \bm{\tau_i}\vert=6$. We use the raised index $\tau_m$ to refer to the $m$-th parameter of the MS ODE plus noise model. For the first parameter of the MS model, we use a Gaussian process prior to encode spatial autocorrelation amongst the values of $\bm{\tau}_1=(\tau_{11},...,\tau_{N1})$ used to parameterize the individual ODE models at $N$ locations. We let $\log \bm{\tau}_1$ denote the elementwise natural logarithm of $\bm{\tau}_1$. The specification for the model's parameters is summarized as

\begin{align*}
    \bm{u}_i &=f_{\bm{\tau}_i}(\bm{x}_i) + \bm{\epsilon}_i\\
    \bm{\epsilon}_i &\sim \mathcal{N}(\bm{0}, \sigma^2_i \bm{I})\\
    %\sigma^2_i &\sim \text{Cauchy}^+(\lambda) \\ 
    \sigma^2_i &\sim \mathcal{N}(0,1)  \\ 
    \log \tau_{im} &\sim \mathcal{N}(\mu_m, s^2_m) \;\; \forall \, i\in\{1,...,N\}, k\in \{2,...,M\}\\
     \log \bm{\tau}_1 &\sim  \mathcal{N}(\bm{\mu}^{(1)}, \bm{K}_{\alpha, \rho})\\
   \alpha &\sim \mathcal{N}(\mu_m, s^2_m) \\ 
    \rho &\sim \text{Uniform}(1,6)\\ 
\end{align*}
\al{Chris, for the log parameters not represented in space, we have to use a different symbol for the variance, right? Because they seem like locations}
\chris{Good catch! Yes, let's use a different parameter. $v$ is a good choice for a variance.}

where we let $\mathcal{N}$ denote a normal distribution 
%and we let $\text{Cauchy}^+$ refer to the half-Cauchy distribution with its mode at zero and with scale parameter $\lambda=XXXX$. 
For reference, a table of notation is presented in Figure XXXX. We assume that the data is measured with additive and independent Gaussian noise, though we allow the intensity of the noise to vary across space. We implement a spatially informed prior distribution for $\bm{\tau}_1$ at locations $\bm{s}_1,...,\bm{s}_N$ by considering these parameter values to be realizations of a random function $\tau_1(\bm{s})$ which has Gaussian process prior

\begin{equation}
\tau_1(\bm{s}) \sim \mathcal{GP}(m(\bm{s}), C(\bm{s}, \bm{s}'; \rho, \alpha))
\end{equation}

where $m(\bm{s}): \mathbb{R}^2\rightarrow \mathbb{R}$ denotes a mean function and $C:\mathbb{R}^2\times \mathbb{R}^2\rightarrow \mathbb{R}$ denotes a suitable covariance kernel function parameterized by a spatial correlation distance parameter $\rho$ and a scale parameter $\alpha$. For simplicity, we model the mean function as a constant value of $m(\bm{s})=\mu_1$ for all values of $\bm{s}\in\mathcal{D}$ Then, the covariance function gives rise to the covariance matrix $K$ via the construction

\begin{equation}
\bm{K}_{\alpha, \rho} = \begin{bmatrix} 
    C(\bm{s}_1, 
\bm{s}_1) &  C(\bm{s}_1, 
\bm{s}_2) & \dots \\
    \vdots & \ddots & \\
     C(\bm{s}_1, 
\bm{s}_N) &        &  C(\bm{s}_N, 
\bm{s}_N)
    \end{bmatrix}
\end{equation}

In this work, we use the squared exponential covariance function, defined as 
\begin{equation}
C(\bm{s}, 
\bm{s}'; \rho, \alpha) = \alpha^2 \exp \left( \frac{ || \bm{s} -\bm{s}'||^2}{2\rho^2} \right)
\end{equation}

where $|| \bm{s} - \bm{s}'||$ denotes the Euclidean distance between two locations $\bm{s}$ and $\bm{s'}$. The role of the correlation distance parameter $\rho$ is to decide roughly how far spatial correlations should extend, while the parameter $\alpha$ determines the relative scale of that variation. We note that this is a standard presentation of Gaussian process priors; we refer the reader to XXXX for more detail. Alternative choices of covariance kernels include the Matern or rational quadratic kernels. If additional spatial structure such as oscillations or trends in space are present, sinusoidal and linear kernels could also be employed. It is important to note that calculating the prior density associated with $\log \bm{\tau}_1$ requires inversion of the pairwise covariance matrix $\bm{K}_{\alpha, \rho}$ which can be numerically unstable. To circumvent this issue, we make use of the Cholesky decomposition $\bm{K}_{\alpha, \rho} = \bm{LL}^T$ within \texttt{Stan}.\\
\par
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
